Regularization for Adversarial Robust Learning

Despite the growing prevalence of artificial neural networks in real-world applications, their vulnerability to adversarial attacks remains a significant concern, which motivates us to investigate the robustness of machine learning models. While various heuristics aim to optimize the distributionally robust risk using the $\infty$-Wasserstein metric, such a notion of robustness frequently encounters computation intractability. To tackle the computational challenge, we develop a novel approach to adversarial training that integrates $\phi$-divergence regularization into the distributionally robust risk function. This regularization brings a notable improvement in computation compared with the original formulation. We develop stochastic gradient methods with biased oracles to solve this problem efficiently, achieving the near-optimal sample complexity. Moreover, we establish its regularization effects and demonstrate it is asymptotic equivalence to a regularized empirical risk minimization framework, by considering various scaling regimes of the regularization parameter and robustness level. These regimes yield gradient norm regularization, variance regularization, or a smoothed gradient norm regularization that interpolates between these extremes. We numerically validate our proposed method in supervised learning, reinforcement learning, and contextual learning and showcase its state-of-the-art performance against various adversarial attacks.

==> arxiv.tex <==
\SingleSpacedXI

\setlength{\parskip}{1ex}
\renewcommand{\theARTICLETOP}{}
\renewcommand{\theARTICLERULE}{\vspace{11pt}}
\renewcommand{\theRRHFirstLine}{}
\renewcommand{\theRRHSecondLine}{}
\renewcommand{\theLRHFirstLine}{}
\renewcommand{\theLRHSecondLine}{}
\renewcommand{\theECLRHFirstLine}{}%
\renewcommand{\theECLRHSecondLine}{}%
\renewcommand{\theECRRHFirstLine}{}%
\renewcommand{\theECRRHSecondLine}{}%
\renewcommand{\endproof}{\endTrivlist\addvspace{2ex}}
\makeatletter
\renewcommand\section{\@startsection {section}{1}{\z@}{-13pt plus -6pt minus -3pt}{4pt}%
  {\fs.13.15.\bfseries\RAGG}}%
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}{-13pt plus -6pt minus -3pt}{4pt}%
  {\TEN\bfseries\RAGG}}%
\makeatother
\let\FigureCaptionFontStyle\undefined
\def\FigureCaptionFontStyle{\mdseries}

\usepackage[scaled=.98,sups,osf,proportional]{XCharter}%


==> premeable.tex <==
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[english]{babel}
\usepackage{microtype}
\usepackage[smallerops,vvarbb]{newtxmath}
\usepackage[varqu,varl]{inconsolata}%
\usepackage[scaled=0.95]{helvet}
\DeclareMathAlphabet{\mathsfit}{T1}{\sfdefault}{\mddefault}{\sldefault}
\SetMathAlphabet{\mathsfit}{bold}{T1}{\sfdefault}{\bfdefault}{\sldefault}
\DeclareMathAlphabet{\mathcal}{OMS}{cmsy}{m}{n}
\usepackage{mathtools,accents}
\usepackage{xifthen,enumitem,comment}
\setlist[enumerate,1]{label=\normalfont{(\Roman*)},leftmargin=2em}
\usepackage{xcolor}
\usepackage{etoolbox}
\makeatletter
\patchcmd{\env@cases}{1.2}{0.96}{}{}
\makeatother
\usepackage{algorithm,algpseudocode}
\usepackage[hypertexnames=false]{hyperref}
\hypersetup{%
  colorlinks=true,%
  linkcolor={blue!66!black},%
  linkbordercolor=red,%
  citecolor={blue!66!black},
}
\usepackage{booktabs,tikz,pgfplots,subfigure}
\usetikzlibrary{matrix,decorations.pathreplacing}

\newcommand{\TBA}{{\color{red}{TBA}}}
\ifx\argmax\undefined\DeclareMathOperator*{\argmax}{arg\,max}\fi
\ifx\argmin\undefined\DeclareMathOperator*{\argmin}{arg\,min}\fi
\DeclareMathOperator*{\esssupOp}{-ess\,sup}
\DeclareMathOperator*{\tsum}{\textstyle{\sum\limits}}
\providecommand\esssup[2]{\underset{#2}{#1\!\esssupOp}}
\providecommand{\Norm}[1]{\lVert\hspace{1pt}#1\hspace{1pt}\rVert}
\providecommand{\norm}[1]{\lVert#1\rVert}
\providecommand{\dist}[2]{\norm{#1-#2}}
\providecommand{\abs}[1]{\lvert#1\rvert}
\providecommand{\diam}{\mathrm{diam}}
\providecommand{\inner}[2]{\left\langle#1,#2\right\rangle}
\providecommand{\Cov}{\mathbb{C}\mathrm{ov}}
\newcommand*{\QED}{%
\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
    \quad\hbox{$\square$}%
}
\newcommand*{\QEG}{%
\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
    \quad\hbox{$\clubsuit$}%
}
\newcommand*{\QDEF}{%
\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
    \quad\hbox{$\diamondsuit$}%
}

\providecommand{\1}{1}
\providecommand{\allOne}{\boldsymbol{1}}
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\hP}{\hat{\mathbb{P}}}
\newcommand{\hx}{\hat{x}}
\newcommand{\hy}{\hat{y}}
\newcommand{\hz}{\hat{z}}
\providecommand{\hxi}{\hat{\xi}}
\providecommand{\hXi}{\hat{\Xi}}
\providecommand{\E}{\mathbb{E}}
\providecommand{\R}{\mathbb{R}}
\providecommand{\CVaR}{\mathbb{C}\textrm{V@R}}
\providecommand{\Var}{\mathbb{V}\textrm{ar}}
\providecommand{\Q}{\mathbb{Q}}
\providecommand{\N}{\mathbb{N}}
\providecommand{\frakM}{\mathfrak{M}}
\providecommand{\cA}{\mathcal{A}}
\providecommand{\cB}{\mathcal{B}}
\providecommand{\cC}{\mathcal{C}}
\providecommand{\cD}{\mathcal{D}}
\providecommand{\cE}{\mathcal{E}}
\providecommand{\cF}{\mathcal{F}}
\providecommand{\cG}{\mathcal{G}}
\providecommand{\cH}{\mathcal{H}}
\providecommand{\cI}{\mathcal{I}}
\providecommand{\cJ}{\mathcal{J}}
\providecommand{\cK}{\mathcal{K}}
\providecommand{\cL}{\mathcal{L}}
\providecommand{\cM}{\mathcal{M}}
\providecommand{\cN}{\mathcal{N}}
\providecommand{\cO}{\mathcal{O}}
\providecommand{\cP}{\mathcal{P}}
\providecommand{\cQ}{\mathcal{Q}}
\providecommand{\cR}{\mathcal{R}}
\providecommand{\cS}{\mathcal{S}}
\providecommand{\cT}{\mathcal{T}}
\providecommand{\cU}{\mathcal{U}}
\providecommand{\cV}{\mathcal{V}}
\providecommand{\cW}{\mathcal{W}}
\providecommand{\cX}{\mathcal{X}}
\providecommand{\cY}{\mathcal{Y}}
\providecommand{\cZ}{\mathcal{Z}}
\providecommand{\bxi}{\boldsymbol{\xi}}
\providecommand{\Rad}{\mathfrak{R}}
\providecommand{\VCdim}{\mathrm{VCdim}}
\providecommand{\Dirac}{\boldsymbol{\updelta}}
\providecommand{\bbsigma}{\boldsymbol{\sigma}}
\providecommand{\tr}{\mathrm{tr}}
\providecommand{\conv}{\mathrm{conv}}

\definecolor{longhorn}{rgb}{0.8, 0.33, 0.0}
\newcommand{\rgao}[1]{{\textcolor{longhorn}{#1}}}
